Towards Repository-Level Program Verification with Large Language Models

Recent advancements in large language models (LLMs) suggest great promises in code and proof generations. However, scaling automated formal verification to real-world projects requires resolving cross-module dependencies and global contexts, which are crucial challenges overlooked by existing LLM-based methods with a special focus on targeting isolated, function-level verification tasks. To systematically explore and address the significant challenges of verifying entire software repositories, we introduce RVBench, the first verification benchmark explicitly designed for repository-level evaluation, constructed from four diverse and complex open-source Verus projects. We further introduce RagVerus, an extensible framework that synergizes retrieval-augmented generation with context-aware prompting to automate proof synthesis for multi-module repositories. RagVerus triples proof pass rates on existing benchmarks under constrained model inference budgets, and achieves a 27% relative improvement on the more challenging RVBench benchmark, demonstrating a scalable and sample-efficient verification solution.

==> code/backup_cd.rs.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{k}{use}\PY{+w}{ }\PY{n}{vstd}::\PY{n}{prelude}::\PY{o}{*}\PY{p}{;}
\PY{k}{fn} \PY{n+nf}{main}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}\PY{p}{\PYZcb{}}
\PY{n}{verus}\PY{o}{!}\PY{p}{\PYZob{}}
\PY{k}{pub}\PY{+w}{ }\PY{k}{fn} \PY{n+nf}{myfun}\PY{p}{(}\PY{n}{a}: \PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{i32}\PY{o}{\PYZgt{}}\PY{p}{,}\PY{+w}{ }\PY{n}{N}: \PY{k+kt}{i32}\PY{p}{)}
\PY{+w}{  }\PY{n}{requires}
\PY{+w}{    }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{    }\PY{n}{old}\PY{p}{(}\PY{n}{a}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{  }\PY{n}{ensures}
\PY{+w}{    }\PY{n}{forall}\PY{+w}{ }\PY{o}{|}\PY{n}{k}:\PY{n+nc}{int}\PY{o}{|}\PY{+w}{ }\PY{l+m+mi}{0}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{o}{=}\PY{+w}{ }\PY{n}{k}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{k}\PY{p}{]}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{p}{,}
\PY{p}{\PYZob{}}
\PY{+w}{  }\PY{k+kd}{let}\PY{+w}{ }\PY{k}{mut}\PY{+w}{ }\PY{n}{i}: \PY{k+kt}{usize} \PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}

\PY{+w}{  }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{  }\PY{p}{\PYZob{}}
\PY{+w}{    }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{;}
\PY{+w}{    }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{  }\PY{p}{\PYZcb{}}

\PY{+w}{  }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{  }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{  }\PY{p}{\PYZob{}}
\PY{+w}{    }\PY{k}{if}\PY{+w}{ }\PY{p}{(}\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{      }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{2}\PY{p}{)}\PY{p}{;}
\PY{+w}{    }\PY{p}{\PYZcb{}}\PY{+w}{ }\PY{k}{else}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{      }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{;}
\PY{+w}{    }\PY{p}{\PYZcb{}}
\PY{+w}{    }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{  }\PY{p}{\PYZcb{}}
\PY{p}{\PYZcb{}}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/backup_ms.rs.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{k}{use}\PY{+w}{ }\PY{n}{vstd}::\PY{n}{prelude}::\PY{o}{*}\PY{p}{;}
\PY{k}{fn} \PY{n+nf}{main}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}\PY{p}{\PYZcb{}}
\PY{n}{verus}\PY{o}{!}\PY{p}{\PYZob{}}

\PY{k}{pub}\PY{+w}{ }\PY{k}{fn} \PY{n+nf}{myfun}\PY{p}{(}\PY{n}{a}: \PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{i32}\PY{o}{\PYZgt{}}\PY{p}{,}\PY{+w}{ }\PY{n}{sum}: \PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{i32}\PY{o}{\PYZgt{}}\PY{p}{,}\PY{+w}{ }\PY{n}{N}: \PY{k+kt}{i32}\PY{p}{)}\PY{+w}{ }
\PY{+w}{  }\PY{n}{requires}\PY{+w}{ }
\PY{+w}{    }\PY{n}{old}\PY{p}{(}\PY{n}{a}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{    }\PY{n}{old}\PY{p}{(}\PY{n}{sum}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{,}
\PY{+w}{    }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{  }\PY{n}{ensures}
\PY{+w}{    }\PY{n}{sum}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{p}{\PYZob{}}
\PY{+w}{  }\PY{k+kd}{let}\PY{+w}{ }\PY{k}{mut}\PY{+w}{ }\PY{n}{i}: \PY{k+kt}{usize} \PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{  }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{  }\PY{p}{\PYZob{}}
\PY{+w}{    }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{)}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{i32}\PY{p}{)}\PY{p}{;}
\PY{+w}{    }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{  }\PY{p}{\PYZcb{}}

\PY{+w}{  }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{  }
\PY{+w}{  }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{  }\PY{p}{\PYZob{}}
\PY{+w}{    }\PY{k}{if}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{      }\PY{n}{sum}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{l+m+mi}{0}\PY{p}{,}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{;}
\PY{+w}{    }\PY{p}{\PYZcb{}}\PY{+w}{ }\PY{k}{else}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{      }\PY{n}{sum}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{l+m+mi}{0}\PY{p}{,}\PY{+w}{ }\PY{n}{sum}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{)}\PY{p}{;}
\PY{+w}{    }\PY{p}{\PYZcb{}}
\PY{+w}{    }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{  }\PY{p}{\PYZcb{}}
\PY{p}{\PYZcb{}}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/cd.rs.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{+w}{  }\PY{l+m+mi}{1}\PY{+w}{ }\PY{k}{use}\PY{+w}{ }\PY{n}{vstd}\PY{p}{::}\PY{n}{prelude}\PY{p}{:}\PY{p}{:}\PY{o}{*}\PY{p}{;}
\PY{+w}{  }\PY{l+m+mi}{2}\PY{+w}{ }\PY{k}{fn}\PY{+w}{ }\PY{n+nf}{main}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}\PY{p}{\PYZcb{}}
\PY{+w}{  }\PY{l+m+mi}{3}\PY{+w}{ }\PY{n}{verus}\PY{o}{!}\PY{p}{\PYZob{}}
\PY{+w}{  }\PY{l+m+mi}{4}\PY{+w}{ }\PY{k}{pub}\PY{+w}{ }\PY{k}{fn}\PY{+w}{ }\PY{n+nf}{myfun}\PY{p}{(}\PY{n}{a}\PY{p}{:}\PY{+w}{ }\PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{i32}\PY{o}{\PYZgt{}}\PY{p}{,}\PY{+w}{ }\PY{n}{N}\PY{p}{:}\PY{+w}{ }\PY{k+kt}{i32}\PY{p}{)}
\PY{+w}{  }\PY{l+m+mi}{5}\PY{+w}{   }\PY{n}{requires}
\PY{+w}{  }\PY{l+m+mi}{6}\PY{+w}{     }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{7}\PY{+w}{     }\PY{n}{old}\PY{p}{(}\PY{n}{a}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{8}
\PY{+w}{  }\PY{l+m+mi}{9}\PY{+w}{   }\PY{n}{ensures}
\PY{+w}{ }\PY{l+m+mi}{10}\PY{+w}{     }\PY{n}{forall}\PY{+w}{ }\PY{o}{|}\PY{n}{k}\PY{p}{:}\PY{n+nc}{int}\PY{o}{|}\PY{+w}{ }\PY{l+m+mi}{0}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{o}{=}\PY{+w}{ }\PY{n}{k}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{k}\PY{p}{]}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{11}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{12}\PY{+w}{   }\PY{k+kd}{let}\PY{+w}{ }\PY{k}{mut}\PY{+w}{ }\PY{n}{i}\PY{p}{:}\PY{+w}{ }\PY{k+kt}{usize}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{13}\PY{+w}{   }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{14}\PY{+w}{     }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{15}\PY{+w}{     }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{16}\PY{+w}{   }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{17}\PY{+w}{   }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{18}\PY{+w}{   }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{19}\PY{+w}{     }\PY{k}{if}\PY{+w}{ }\PY{p}{(}\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{20}\PY{+w}{       }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{2}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{21}\PY{+w}{     }\PY{p}{\PYZcb{}}\PY{+w}{ }\PY{k}{else}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{22}\PY{+w}{       }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{23}\PY{+w}{     }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{24}\PY{+w}{     }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{25}\PY{+w}{   }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{26}\PY{+w}{ }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{27}\PY{+w}{ }\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/cd_verified.rs.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{+w}{  }\PY{l+m+mi}{1}\PY{+w}{ }\PY{k}{use}\PY{+w}{ }\PY{n}{vstd}\PY{p}{::}\PY{n}{prelude}\PY{p}{:}\PY{p}{:}\PY{o}{*}\PY{p}{;}
\PY{+w}{  }\PY{l+m+mi}{2}\PY{+w}{ }\PY{k}{fn}\PY{+w}{ }\PY{n+nf}{main}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}\PY{p}{\PYZcb{}}
\PY{+w}{  }\PY{l+m+mi}{3}\PY{+w}{ }\PY{n}{verus}\PY{o}{!}\PY{p}{\PYZob{}}
\PY{+w}{  }\PY{l+m+mi}{4}\PY{+w}{ }\PY{k}{pub}\PY{+w}{ }\PY{k}{fn}\PY{+w}{ }\PY{n+nf}{myfun}\PY{p}{(}\PY{n}{a}\PY{p}{:}\PY{+w}{ }\PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{i32}\PY{o}{\PYZgt{}}\PY{p}{,}\PY{+w}{ }\PY{n}{N}\PY{p}{:}\PY{+w}{ }\PY{k+kt}{u32}\PY{p}{)}
\PY{+w}{  }\PY{l+m+mi}{5}\PY{+w}{   }\PY{n}{requires}
\PY{+w}{  }\PY{l+m+mi}{6}\PY{+w}{     }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{7}\PY{+w}{     }\PY{n}{old}\PY{p}{(}\PY{n}{a}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{8}
\PY{+w}{  }\PY{l+m+mi}{9}\PY{+w}{   }\PY{n}{ensures}
\PY{+w}{ }\PY{l+m+mi}{10}\PY{+w}{     }\PY{n}{forall}\PY{+w}{ }\PY{o}{|}\PY{n}{k}\PY{p}{:}\PY{n+nc}{int}\PY{o}{|}\PY{+w}{ }\PY{l+m+mi}{0}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{o}{=}\PY{+w}{ }\PY{n}{k}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{k}\PY{p}{]}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{11}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{12}\PY{+w}{   }\PY{k+kd}{let}\PY{+w}{ }\PY{k}{mut}\PY{+w}{ }\PY{n}{i}\PY{p}{:}\PY{+w}{ }\PY{k+kt}{usize}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{13}\PY{+w}{   }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{ }\PY{l+m+mi}{14}\PY{+w}{     }\PY{n}{invariant}
\PY{+w}{ }\PY{l+m+mi}{15}\PY{+w}{       }\PY{n}{forall}\PY{+w}{ }\PY{o}{|}\PY{n}{k}\PY{p}{:}\PY{n+nc}{int}\PY{o}{|}\PY{+w}{ }\PY{l+m+mi}{0}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{o}{=}\PY{+w}{ }\PY{n}{k}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{k}\PY{p}{]}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{16}\PY{+w}{       }\PY{n}{a}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{17}\PY{+w}{   }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{18}\PY{+w}{     }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{19}\PY{+w}{     }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{20}\PY{+w}{   }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{21}\PY{+w}{   }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{22}\PY{+w}{   }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{ }\PY{l+m+mi}{23}\PY{+w}{     }\PY{n}{invariant}
\PY{+w}{ }\PY{l+m+mi}{24}\PY{+w}{       }\PY{n}{forall}\PY{+w}{ }\PY{o}{|}\PY{n}{k}\PY{p}{:}\PY{n+nc}{int}\PY{o}{|}\PY{+w}{ }\PY{l+m+mi}{0}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{o}{=}\PY{+w}{ }\PY{n}{k}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{k}\PY{p}{]}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{25}\PY{+w}{       }\PY{n}{forall}\PY{+w}{ }\PY{o}{|}\PY{n}{k}\PY{p}{:}\PY{n+nc}{int}\PY{o}{|}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{o}{=}\PY{+w}{ }\PY{n}{k}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{k}\PY{p}{]}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{26}\PY{+w}{       }\PY{n}{a}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{27}
\PY{+w}{ }\PY{l+m+mi}{28}\PY{+w}{   }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{29}\PY{+w}{     }\PY{k}{if}\PY{+w}{ }\PY{p}{(}\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{2}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{30}\PY{+w}{       }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{2}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{31}\PY{+w}{     }\PY{p}{\PYZcb{}}\PY{+w}{ }\PY{k}{else}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{32}\PY{+w}{       }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{33}\PY{+w}{     }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{34}\PY{+w}{     }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{35}\PY{+w}{   }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{36}\PY{+w}{ }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{37}\PY{+w}{ }\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\@namedef{PY@tok@w}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\@namedef{PY@tok@c}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cp}{\def\PY@tc##1{\textcolor[rgb]{0.61,0.40,0.00}{##1}}}
\@namedef{PY@tok@k}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kp}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kt}{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\@namedef{PY@tok@o}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@ow}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PY@tok@nb}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@nf}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@nc}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@nn}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@ne}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.80,0.25,0.22}{##1}}}
\@namedef{PY@tok@nv}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@no}{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\@namedef{PY@tok@nl}{\def\PY@tc##1{\textcolor[rgb]{0.46,0.46,0.00}{##1}}}
\@namedef{PY@tok@ni}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PY@tok@na}{\def\PY@tc##1{\textcolor[rgb]{0.41,0.47,0.13}{##1}}}
\@namedef{PY@tok@nt}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@nd}{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PY@tok@s}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sd}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@si}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PY@tok@se}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.36,0.12}{##1}}}
\@namedef{PY@tok@sr}{\def\PY@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PY@tok@ss}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@sx}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@m}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@gh}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PY@tok@gu}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\@namedef{PY@tok@gd}{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\@namedef{PY@tok@gi}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.52,0.00}{##1}}}
\@namedef{PY@tok@gr}{\def\PY@tc##1{\textcolor[rgb]{0.89,0.00,0.00}{##1}}}
\@namedef{PY@tok@ge}{\let\PY@it=\textit}
\@namedef{PY@tok@gs}{\let\PY@bf=\textbf}
\@namedef{PY@tok@gp}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PY@tok@go}{\def\PY@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PY@tok@gt}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\@namedef{PY@tok@err}{\def\PY@bc##1{{\setlength{\fboxsep}{\string -\fboxrule}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}}
\@namedef{PY@tok@kc}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kd}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kn}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kr}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@bp}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@fm}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@vc}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vg}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vi}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vm}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@sa}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sb}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sc}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@dl}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@s2}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sh}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@s1}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@mb}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mf}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mh}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mi}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@il}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mo}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@ch}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cm}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cpf}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@c1}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cs}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/ms.rs.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{+w}{  }\PY{l+m+mi}{1}\PY{+w}{ }\PY{k}{use}\PY{+w}{ }\PY{n}{vstd}\PY{p}{::}\PY{n}{prelude}\PY{p}{:}\PY{p}{:}\PY{o}{*}\PY{p}{;}
\PY{+w}{  }\PY{l+m+mi}{2}\PY{+w}{ }\PY{k}{fn}\PY{+w}{ }\PY{n+nf}{main}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}\PY{p}{\PYZcb{}}
\PY{+w}{  }\PY{l+m+mi}{3}\PY{+w}{ }\PY{n}{verus}\PY{o}{!}\PY{p}{\PYZob{}}
\PY{+w}{  }\PY{l+m+mi}{4}\PY{+w}{ }\PY{k}{pub}\PY{+w}{ }\PY{k}{fn}\PY{+w}{ }\PY{n+nf}{myfun}\PY{p}{(}\PY{n}{a}\PY{p}{:}\PY{+w}{ }\PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{i32}\PY{o}{\PYZgt{}}\PY{p}{,}\PY{+w}{ }\PY{n}{sum}\PY{p}{:}\PY{+w}{ }\PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{i32}\PY{o}{\PYZgt{}}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{5}\PY{+w}{   }\PY{n}{requires}
\PY{+w}{  }\PY{l+m+mi}{6}\PY{+w}{     }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{7}\PY{+w}{     }\PY{n}{old}\PY{p}{(}\PY{n}{a}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{8}\PY{+w}{     }\PY{n}{old}\PY{p}{(}\PY{n}{sum}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{9}\PY{+w}{   }\PY{n}{ensures}
\PY{+w}{ }\PY{l+m+mi}{10}\PY{+w}{     }\PY{n}{sum}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{11}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{12}\PY{+w}{   }\PY{k+kd}{let}\PY{+w}{ }\PY{k}{mut}\PY{+w}{ }\PY{n}{i}\PY{p}{:}\PY{+w}{ }\PY{k+kt}{usize}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{13}\PY{+w}{   }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{14}\PY{+w}{     }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{)}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{i32}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{15}\PY{+w}{     }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{16}\PY{+w}{   }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{17}\PY{+w}{   }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{18}\PY{+w}{   }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{19}\PY{+w}{     }\PY{k}{if}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{20}\PY{+w}{       }\PY{n}{sum}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{l+m+mi}{0}\PY{p}{,}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{21}\PY{+w}{     }\PY{p}{\PYZcb{}}\PY{+w}{ }\PY{k}{else}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{22}\PY{+w}{       }\PY{n}{sum}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{l+m+mi}{0}\PY{p}{,}\PY{+w}{ }\PY{n}{sum}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{23}\PY{+w}{     }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{24}\PY{+w}{     }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{25}\PY{+w}{   }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{26}\PY{+w}{ }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{27}\PY{+w}{ }\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/ms_verified.rs.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{+w}{  }\PY{l+m+mi}{1}\PY{+w}{ }\PY{k}{use}\PY{+w}{ }\PY{n}{vstd}\PY{p}{::}\PY{n}{prelude}\PY{p}{:}\PY{p}{:}\PY{o}{*}\PY{p}{;}
\PY{+w}{  }\PY{l+m+mi}{2}\PY{+w}{ }\PY{k}{fn}\PY{+w}{ }\PY{n+nf}{main}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}\PY{p}{\PYZcb{}}
\PY{+w}{  }\PY{l+m+mi}{3}\PY{+w}{ }\PY{n}{verus}\PY{o}{!}\PY{p}{\PYZob{}}
\PY{+w}{  }\PY{l+m+mi}{4}\PY{+w}{ }\PY{k}{pub}\PY{+w}{ }\PY{k}{fn}\PY{+w}{ }\PY{n+nf}{myfun}\PY{p}{(}\PY{n}{a}\PY{p}{:}\PY{+w}{ }\PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{usize}\PY{o}{\PYZgt{}}\PY{p}{,}\PY{+w}{ }\PY{n}{sum}\PY{p}{:}\PY{+w}{ }\PY{k+kp}{\PYZam{}}\PY{n+nc}{mut}\PY{+w}{ }\PY{n+nb}{Vec}\PY{o}{\PYZlt{}}\PY{k+kt}{usize}\PY{o}{\PYZgt{}}\PY{p}{,}\PY{+w}{ }\PY{n}{N}\PY{p}{:}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{  }\PY{l+m+mi}{5}\PY{+w}{   }\PY{n}{requires}
\PY{+w}{  }\PY{l+m+mi}{6}\PY{+w}{     }\PY{n}{N}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{7}\PY{+w}{     }\PY{n}{old}\PY{p}{(}\PY{n}{a}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{8}\PY{+w}{     }\PY{n}{old}\PY{p}{(}\PY{n}{sum}\PY{p}{)}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{,}
\PY{+w}{  }\PY{l+m+mi}{9}\PY{+w}{   }\PY{n}{ensures}
\PY{+w}{ }\PY{l+m+mi}{10}\PY{+w}{     }\PY{n}{sum}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{11}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{12}\PY{+w}{   }\PY{k+kd}{let}\PY{+w}{ }\PY{k}{mut}\PY{+w}{ }\PY{n}{i}\PY{p}{:}\PY{+w}{ }\PY{k+kt}{usize}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{13}\PY{+w}{   }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{ }\PY{l+m+mi}{14}\PY{+w}{     }\PY{n}{invariant}
\PY{+w}{ }\PY{l+m+mi}{15}\PY{+w}{       }\PY{n}{forall}\PY{+w}{ }\PY{o}{|}\PY{n}{k}\PY{p}{:}\PY{+w}{ }\PY{n+nc}{int}\PY{o}{|}\PY{+w}{ }\PY{l+m+mi}{0}\PY{o}{\PYZlt{}}\PY{o}{=}\PY{+w}{ }\PY{n}{k}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{k}\PY{p}{]}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{16}\PY{+w}{       }\PY{n}{a}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{17}\PY{+w}{   }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{18}\PY{+w}{     }\PY{n}{a}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{n}{i}\PY{p}{,}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZpc{}}\PY{+w}{ }\PY{l+m+mi}{1}\PY{+w}{ }\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{19}\PY{+w}{     }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{20}\PY{+w}{   }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{21}\PY{+w}{   }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{22}\PY{+w}{   }\PY{k}{while}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{k}{as}\PY{+w}{ }\PY{k+kt}{usize}\PY{p}{)}
\PY{+w}{ }\PY{l+m+mi}{23}\PY{+w}{     }\PY{n}{invariant}
\PY{+w}{ }\PY{l+m+mi}{24}\PY{+w}{       }\PY{n}{forall}\PY{+w}{ }\PY{o}{|}\PY{n}{k}\PY{p}{:}\PY{+w}{ }\PY{n+nc}{int}\PY{o}{|}\PY{+w}{ }\PY{l+m+mi}{0}\PY{o}{\PYZlt{}}\PY{o}{=}\PY{+w}{ }\PY{n}{k}\PY{+w}{ }\PY{o}{\PYZlt{}}\PY{+w}{ }\PY{n}{N}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{k}\PY{p}{]}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{25}\PY{+w}{       }\PY{n}{a}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{n}{N}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{26}\PY{+w}{       }\PY{n}{i}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{l+m+mi}{0}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{sum}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{27}\PY{+w}{       }\PY{n}{sum}\PY{p}{.}\PY{n}{len}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{,}
\PY{+w}{ }\PY{l+m+mi}{28}\PY{+w}{   }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{29}\PY{+w}{     }\PY{k}{if}\PY{+w}{ }\PY{p}{(}\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{o}{=}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{30}\PY{+w}{       }\PY{n}{sum}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{l+m+mi}{0}\PY{p}{,}\PY{+w}{ }\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{31}\PY{+w}{     }\PY{p}{\PYZcb{}}\PY{+w}{ }\PY{k}{else}\PY{+w}{ }\PY{p}{\PYZob{}}
\PY{+w}{ }\PY{l+m+mi}{32}\PY{+w}{       }\PY{n}{sum}\PY{p}{.}\PY{n}{set}\PY{p}{(}\PY{l+m+mi}{0}\PY{p}{,}\PY{+w}{ }\PY{n}{sum}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{n}{a}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{)}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{33}\PY{+w}{     }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{34}\PY{+w}{     }\PY{n}{i}\PY{+w}{ }\PY{o}{=}\PY{+w}{ }\PY{n}{i}\PY{+w}{ }\PY{o}{+}\PY{+w}{ }\PY{l+m+mi}{1}\PY{p}{;}
\PY{+w}{ }\PY{l+m+mi}{35}\PY{+w}{   }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{36}\PY{+w}{ }\PY{p}{\PYZcb{}}
\PY{+w}{ }\PY{l+m+mi}{37}\PY{+w}{ }\PY{p}{\PYZcb{}}
\end{Verbatim}

